OAMixer: Object-aware Mixing Layer for Vision Transformers

Patch-based models, e.g., Vision Transformers (ViTs) and Mixers, have shown impressive results on various visual recognition tasks, alternating classic convolutional networks. While the initial patch-based models (ViTs) treated all patches equally, recent studies reveal that incorporating inductive bias like spatiality benefits the representations. However, most prior works solely focused on the location of patches, overlooking the scene structure of images. Thus, we aim to further guide the interaction of patches using the object information. Specifically, we propose OAMixer (object-aware mixing layer), which calibrates the patch mixing layers of patch-based models based on the object labels. Here, we obtain the object labels in unsupervised or weakly-supervised manners, i.e., no additional human-annotating cost is necessary. Using the object labels, OAMixer computes a reweighting mask with a learnable scale parameter that intensifies the interaction of patches containing similar objects and applies the mask to the patch mixing layers. By learning an object-centric representation, we demonstrate that OAMixer improves the classification accuracy and background robustness of various patch-based models, including ViTs, MLP-Mixers, and ConvMixers. Moreover, we show that OAMixer enhances various downstream tasks, including large-scale classification, self-supervised learning, and multi-object recognition, verifying the generic applicability of OAMixer

==> _cvprw2022_(arxiv)/resources/fig_concept.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=.9\textwidth]{figures/concept.pdf}
\caption{
Conceptual illustration of our method, OAMixer. Given an image $\x$, we assume that patch-wise object labels $\y$ (either from pixel-level labels or given by patch-level directly) are available. Using this label, we compute a reweighting mask $\M$ which modifies the original patch mixing layer $f_\texttt{mix}$ to the data-specific \textit{object-aware mixed} layer $f_\texttt{oamix}$.
}\label{fig:concept}
\end{figure*}




==> _cvprw2022_(arxiv)/resources/fig_mixing.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}{0.28\textwidth}
\includegraphics[width=\textwidth]{figures/attn.png}
\caption{Self-attention}
\end{subfigure}
\begin{subfigure}{0.28\textwidth}
\includegraphics[width=\textwidth]{figures/mlp.png}
\caption{Feed-forward}
\end{subfigure}
\begin{subfigure}{0.28\textwidth}
\includegraphics[width=\textwidth]{figures/conv.png}
\caption{Convolution}
\end{subfigure}
\caption{
Illustration of representative patch mixing layers $f_\texttt{mix}$: (a) self-attention, (b) feed-forward, and (c) convolution. All layers map $N$ input patches to $N$ output patches, updating the values by interacting among the patches.
}\label{fig:mixing}
\end{figure*}




==> _cvprw2022_(arxiv)/resources/fig_saliency.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}{0.13\textwidth}
\includegraphics[width=\textwidth]{figures/saliency_orig.png}
\caption{Original}
\end{subfigure}
\begin{subfigure}{0.13\textwidth}
\includegraphics[width=\textwidth]{figures/saliency_base.png}
\caption{DeiT-S}
\end{subfigure}
\begin{subfigure}{0.13\textwidth}
\includegraphics[width=\textwidth]{figures/saliency_ours.png}
\caption{OAMixer}
\end{subfigure}
\caption{
Saliency maps of DeiT-S and OAMixer (ours).
}\label{fig:saliency}
%\vspace{-0.02in}
\end{figure}

==> _cvprw2022_(arxiv)/resources/tab_bg_challenge.tex <==
\begin{table*}[t]
\caption{
Comparison of various scenarios evaluated on the Background Challenge benchmark. We report the classification accuracy (\buparrow) and background robustness (\rdownarrow), where higher and lower values are better for each metric. ``TL'' indicates TokenLabeling, that the model is trained with an additional token-level objective. Note that TL improves the overall performance; we colored them with gray lines for better visualization. We use ReLabel from ImageNet trained model for both OAMixer and TL. `+' denotes the modules added to the baseline (not accumulated), and parenthesis denotes the gap from the baseline. The table has several implications: (a) OAMixer consistently improves the classification and background robustness, confirming the benefit of object-centric representation. (b) OAMixer outperforms the methods using spatial inductive bias like ConViT and CoAtNet; combining ConViT and OAMixer performs even better. (c) OAMixer gives additional gain over TL, verifying the merit of guided patch interaction over na\"ive patch-level objective. (d) OAMixer also improves MLP-Mixer and ConvMixer, patch-based models using different patch mixing layers.
}\label{tab:bg}
\centering%\small
% \resizebox{\textwidth}{!}{% 
\begin{tabular}{lclllll}
\toprule
& TL & Original (\buparrow) & Only-BG-B (\rdownarrow) & Mixed-Same (\buparrow) & Mixed-Rand (\buparrow) & BG-Gap (\rdownarrow)\\
\midrule
DeiT-T           & - & 70.62 & 35.48 & 63.31 & 39.56 & 23.75 \\
+ ConViT         & - & 78.74 \bup{8.12} & 38.69 \bup{3.21} & 70.84 \bup{7.53} & 46.91 \bup{7.35} & 23.93 \bup{0.18}  \\
+ CoAtNet        & - & 78.62 \bup{8.00} & 37.68 \bup{2.20} & 70.40 \bup{7.09} & 45.46 \bup{5.90} & 24.94 \bup{1.19}  \\
+ OAMixer (ours) & - & 81.98 \bup{11.36} & 30.89 \rdown{4.59} & 73.38 \bup{10.07} & 51.53 \bup{11.97} & 21.85 \rdown{1.90}  \\
+ OAMixer + ConViT (ours) & - & 83.38 \bup{12.76} & 31.36 \rdown{4.12} & 74.86 \bup{11.55} & 53.14 \bup{13.58} & 21.73 \rdown{2.02}  \\
\rowcolor{lightgray}
DeiT-T           & \checkmark & 83.50 & 37.01 & 74.57 & 51.78 & 22.79 \\
\rowcolor{lightgray}
+ OAMixer (ours) & \checkmark & 87.23 \bup{3.73} & 29.21 \rdown{7.80} & 78.15 \bup{3.58} & 60.59 \bup{8.81} & 17.56 \rdown{5.23} \\
\midrule
DeiT-S           & - & 82.69 & 39.46 & 73.88 & 50.49 & 23.39\\
+ ConViT         & - & 85.51 \bup{2.82} & 38.94 \rdown{0.52} & 76.40 \bup{2.52} & 54.37 \bup{3.88} & 22.03 \rdown{1.36}  \\
+ OAMixer (ours) & - & 86.32 \bup{3.63} & 31.78 \rdown{7.68} & 78.44 \bup{4.56} & 56.74 \bup{6.25} & 21.70 \rdown{1.69}  \\
+ OAMixer + ConViT (ours) & - & 88.20 \bup{5.51} & 30.79 \rdown{8.67} & 79.16 \bup{5.28} & 60.52 \bup{10.03} & 18.64 \rdown{4.75}  \\
\rowcolor{lightgray}
DeiT-S           & \checkmark & 88.52 & 38.00 & 79.43 & 59.36 & 20.07 \\
\rowcolor{lightgray}
+ OAMixer (ours) & \checkmark & 91.31 \bup{2.79} & 29.19 \rdown{8.81} & 81.78 \bup{2.35} & 66.92 \bup{7.56} & 14.86 \rdown{5.21} \\
\midrule
MLP-Mixer-S/16   & - & 84.99 & 40.96 & 76.52 & 54.72 & 21.80\\
+ OAMixer (ours) & - & 87.68 \bup{2.69} & 27.28 \rdown{13.68} & 79.43 \bup{2.91} & 60.44 \bup{5.72} & 18.99 \rdown{2.81}  \\
\rowcolor{lightgray}
MLP-Mixer-S/16   & \checkmark & 88.07 & 38.17 & 79.21 & 58.72 & 20.49 \\
\rowcolor{lightgray}
+ OAMixer (ours) & \checkmark & 90.49 \bup{2.42} & 28.72 \rdown{9.45} & 81.63 \bup{2.42} & 65.36 \bup{6.64} & 16.27 \rdown{4.22} \\
\midrule
ConvMixer-S/16   & - & 86.32 & 41.38 & 78.59 & 56.99 & 21.60\\
+ OAMixer (ours) & - & 88.49 \bup{2.17} & 35.60 \rdown{5.78} & 81.70 \bup{3.11} & 63.93 \bup{6.94} & 17.77 \rdown{3.83}  \\
\rowcolor{lightgray}
ConvMixer-S/16   & \checkmark & 87.49 & 36.49 & 80.42 & 58.15 & 22.27 \\
\rowcolor{lightgray}
+ OAMixer (ours) & \checkmark & 89.09 \bup{1.60} & 32.67 \rdown{3.82} & 82.64 \bup{2.22} & 63.70 \bup{5.55} & 18.94 \rdown{3.33}\\
\bottomrule
\end{tabular}
\end{table*}




==> _cvprw2022_(arxiv)/resources/tab_cls_imagenet.tex <==
\begin{table*}[t]
\caption{
ImageNet top-1 accuracy. We add TokenLabeling (TL) and OAMixer on top of the baseline models (accumulated). Both TL and OAMixer use ReLabel object labels from ImageNet-trained model. Bold denotes the best result, and parenthesis denotes the gap from the baseline. Note that TL requires enough model capacity (better for the larger model, even harms MobileViT-XXS). In contrast, OAMixer gives a consistent improvement over all considered model capacities.
}\label{tab:cls-imagenet}
\centering%\small
% \resizebox{0.7\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
& MobileViT-XXS & DeiT-T & DeiT-S & DeiT-B \\
\midrule
\# params & 1.3M & 5M & 22M & 86M \\
\midrule
Baseline & 62.56 \blank & 71.19 \blank & 79.30 \blank & 78.45 \blank \\
+ TokenLabeling & 62.34 \down{0.22} & 71.61 \up{0.42} & 80.20 \up{0.90} & 81.17 \up{2.72} \\
+ OAMixer (ours) & \textbf{64.78} \up{2.22} & \textbf{74.26} \up{3.07} & \textbf{81.26} \up{1.96} & \textbf{82.18} \up{3.73} \\
\bottomrule
\end{tabular}
% }
\end{table*}


==> _cvprw2022_(arxiv)/resources/tab_cls_more.tex <==
\begin{table*}[t]
\caption{
Classification accuracy on various datasets. We add OAMixer to the baseline models, where ``OAMixer'' uses ReLabel trained on each downstream dataset, and ``OAMixer$^*$'' uses ReLabel trained on ImageNet. Bold denotes the best result among methods not using ImageNet data (not colored by gray lines), and parenthesis denotes the gap from the baseline. OAMixer gives a consistent improvement, showing comparable results with OAMixer$^*$ for all considered datasets.
}\label{tab:cls-more}
% \vspace{-0.08in}
\centering%\small
% \resizebox{0.8\textwidth}{!}{%
\begin{tabular}{lccgccg}
\toprule
& \multicolumn{3}{c}{DeiT-T} & \multicolumn{3}{c}{DeiT-S} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7} 
& Baseline & OAMixer (ours) & OAMixer$^*$ (ours) & Baseline & OAMixer (ours) & OAMixer$^*$ (ours) \\
\midrule
CIFAR-10  & 86.35 & \textbf{89.89} \up{3.54} & 88.09 \up{1.74} & 90.80 & \textbf{92.73} \up{1.93} & 92.33 \up{1.53} \\
CIFAR-100 & 65.21 & \textbf{66.94} \up{1.73} & 67.21 \up{2.00} & 70.08 & \textbf{71.00} \up{0.92} & 71.63 \up{1.55} \\
Food-101  & 69.83 & \textbf{72.25} \up{2.42} & 71.50 \up{1.67} & 75.00 & \textbf{75.17} \up{0.17} & 76.03 \up{1.03} \\
Pets & 24.20 & \textbf{24.50} \up{0.30} & 24.97 \up{0.57} & 25.57 & \textbf{30.64} \up{5.07} & 29.63 \up{4.06} \\
\bottomrule
\end{tabular}
% }
\end{table*}

==> _cvprw2022_(arxiv)/resources/tab_cls_multi.tex <==
\begin{table}[t]
\caption{
%Mean average precision (mAP) for multi-object recognition on the COCO dataset. We add OAMixer on top of the baseline models, where the object labels are given by ReLabel trained on ImageNet. Bold denotes the best results, and parenthesis denotes the gap from the baseline. OAMixer improves all considered scenarios, verifying its effectiveness on the multi-object images.
Mean average precision (mAP) for multi-object recognition on the COCO dataset. We use the patch-wise object labels, which are given by ReLabel trained on ImageNet. Bold denotes the best results, and parenthesis denotes the gap from the baseline. OAMixer is also effective for recognizing multi-object images.
% all considered scenarios, verifying its effectiveness on the multi-object images.
}\label{tab:cls-multi}
% \vspace{-0.08in}
\centering\small
% \resizebox{0.7\textwidth}{!}{%
\begin{tabular}{cccc}
\toprule
\multicolumn{2}{c}{DeiT-T} & \multicolumn{2}{c}{DeiT-S} \\
\cmidrule(lr){1-2}\cmidrule(lr){3-4} 
Baseline & OAMixer (ours) & Baseline & OAMixer (ours) \\
\midrule
57.42 & \textbf{59.56} \up{2.14} & 60.93 & \textbf{62.23} \up{1.30} \\
\bottomrule
\end{tabular}%}
\end{table}

==> _cvprw2022_(arxiv)/resources/tab_dino.tex <==
\begin{table*}[t]
\caption{
Linear probing results of DINO with DeiT-T trained on ImageNet with 100 epochs. We use the unsupervised attention map from the pretrained baseline DINO model as a patch-wise object label for OAMixer. We test the in-domain accuracy with the ImageNet validation dataset and out-domain accuracy with Background Challenge datasets after training the linear classifier on the ImageNet train set with 100 epochs. The results show that OAMixer is effective in the self-supervised framework.
}\label{tab:dino}
\centering%\small
% \resizebox{0.8\textwidth}{!}{% 
\begin{tabular}{llllll}
\toprule
& ImageNet (\buparrow) & Only-BG-B (\rdownarrow) & Mixed-Same (\buparrow) & Mixed-Rand (\buparrow) & BG-Gap (\rdownarrow)\\
\midrule
DeiT-T            & 59.37 & 34.27 & 89.73 & 78.07 & 11.66 \\
+ OAMixer          & 61.16 \bup{1.79} & 20.20 \rdown{14.07} & 89.75 \bup{0.02} & 79.33 \bup{1.26} & 10.42 \rdown{1.24} \\
\bottomrule
\end{tabular}
% }
\end{table*}




==> _cvprw2022_(arxiv)/resources/tab_dist_shift.tex <==
\begin{table*}[t]
\caption{
Classification accuracy on various distribution-shifted datasets. Bold denotes the best results, and parenthesis denotes the gap from the baseline. OAMixer gives consistent improvements.
}\label{tab:dist-shift}
\centering%\small
% \resizebox{0.7\textwidth}{!}{% 
\begin{tabular}{ll|lllll}
\toprule
& ImageNet-9 & ImageNetV2-9 & ReaL-9 & Rendition-9 & Stylized-9 & Sketch-9 \\
\midrule
DeiT-T           & 70.62 & 63.19 & 68.13 & 24.14 & 16.66 & 21.65 \\
+ OAMixer (ours) & \textbf{80.15} \up{9.53} & \textbf{70.68} \up{7.49} & \textbf{77.78} \up{9.65} & \textbf{27.53} \up{3.39} & \textbf{21.80} \up{5.14} & \textbf{24.45} \up{2.80} \\
\midrule
DeiT-S           & 82.69 & 73.22 & 80.21 & 28.60 & 21.90 & 27.26 \\
+ OAMixer (ours) & \textbf{83.88} \up{1.19} & \textbf{75.68} \up{2.46} & \textbf{82.37} \up{2.16} & \textbf{29.43} \up{0.83} & \textbf{24.64} \up{2.74} & \textbf{27.93} \up{0.67} \\
% \midrule
% MLP-Mixer-S/32   & 75.73 & 64.92 & 71.35 & 27.60 & 20.77 & 23.38 \\
% + OAMixer (ours) & \textbf{77.36} \up{1.63} & \textbf{66.00} \up{1.08} & \textbf{72.82} \up{1.47} & \textbf{28.24} \up{0.64} & \textbf{21.50} \up{0.73} & \textbf{25.49} \up{2.11} \\
%\midrule
%MLP-Mixer-S/16   & 84.99 & \textbf{76.57} & 82.70 & 34.25 & 25.54 & 37.07 \\
%+ OAMixer (ours) & \textbf{86.30} \up{1.31} & 76.51 \down{0.06} & \textbf{83.37} \up{0.67} & \textbf{34.29} \up{0.04} & \textbf{27.08} \up{1.54} & \textbf{38.16} \up{1.09} \\
% \midrule
% ConvMixer-S/32   & 77.33 & 68.32 & 74.63 & 28.88 & 20.80 & 25.59 \\
% + OAMixer (ours) & \textbf{77.73} \up{0.40} & \textbf{68.73} \up{0.41} & \textbf{74.78} \up{0.15} & \textbf{30.87} \up{1.99} & \textbf{21.29} \up{0.49} & \textbf{31.45} \up{5.86} \\
%\midrule
%ConvMixer-S/16   & 86.32 & 76.38 & 83.16 & 33.33 & 24.21 & 34.36 \\
%+ OAMixer (ours) & \textbf{86.35} \up{0.03} & \textbf{76.97} \up{0.59} & \textbf{83.56} \up{0.40} & \textbf{33.81} \up{0.48} & \textbf{24.94} \up{0.73} & \textbf{35.72} \up{1.36} \\
\bottomrule
\end{tabular}
\end{table*}


==> _cvprw2022_(arxiv)/resources/tab_dist_shift_summary.tex <==
\begin{table}[t]
\caption{
sss
}\label{tab:dist-shift-summary}
% \vspace{-0.08in}
\centering\small
% \resizebox{0.7\textwidth}{!}{%
\begin{tabular}{cccc}
\toprule
\multicolumn{2}{c}{DeiT-T} & \multicolumn{2}{c}{DeiT-S} \\
\cmidrule(lr){1-2}\cmidrule(lr){3-4} 
Baseline & OAMixer (ours) & Baseline & OAMixer (ours) \\
\midrule
57.42 & \textbf{59.56} \up{2.14} & 60.93 & \textbf{62.23} \up{1.30} \\
\bottomrule
\end{tabular}%}
\end{table}

==> _cvprw2022_(arxiv)/resources/tab_mask_scale.tex <==
\begin{table*}[t]
\begin{minipage}{0.48\textwidth}
\captionof{table}{
Learned mask scales $\kappa^{(l)}$ over layers.
}\label{tab:mask-scale}
%\vspace{-0.08in}
\resizebox{\textwidth}{!}{% 
\begin{tabular}{lcccc}
\toprule
& Layer 1/4 & Layer 2/4 & Layer 3/4 & Layer 4/4 \\
\midrule
DeiT-S         & 1.571 & 0.783 & 0.945 & 0.287 \\
MLP-Mixer-S/16 & 0.744 & 0.000 & 0.001 & 0.061 \\
ConvMixer-S/16 & 0.871 & 2.347 & 1.498 & 0.001 \\
\bottomrule
\end{tabular}}
\end{minipage}~~~~
\begin{minipage}{0.38\textwidth}
\centering
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/saliency_orig.png}
\caption{Original}
\end{subfigure}~
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/saliency_base.png}
\caption{DeiT-S}
\end{subfigure}~
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/saliency_ours.png}
\caption{OAMixer}
\end{subfigure}
%\vspace{-0.05in}
\captionof{figure}{
Saliency map visualization.
}\label{fig:saliency}
\end{minipage}
\end{table*}




==> _cvprw2022_(arxiv)/resources/tab_mask_scale_only.tex <==
\begin{table}[t]
%\vspace{-0.02in}
\captionof{table}{
Learned mask scales $\kappa^{(l)}$ over layers.
}\label{tab:mask-scale}
\centering%\small
\resizebox{.95\linewidth}{!}{% 
\begin{tabular}{lcccc}
\toprule
& Layer 1/4 & Layer 2/4 & Layer 3/4 & Layer 4/4 \\
\midrule
% DeiT-S         & 1.57 & 0.78 & 0.95 & 0.29 \\
% MLP-Mixer-S/16 & 0.74 & 0.00 & 0.00 & 0.06 \\
% ConvMixer-S/16 & 0.87 & 2.35 & 1.50 & 0.00 \\
DeiT-S         & 1.571 & 0.783 & 0.945 & 0.287 \\
MLP-Mixer-S/16 & 0.744 & 0.000 & 0.001 & 0.061 \\
ConvMixer-S/16 & 0.871 & 2.347 & 1.498 & 0.001 \\
\bottomrule
\end{tabular}}
%\vspace{-0.02in}
\end{table}




==> _cvprw2022_(arxiv)/resources/tab_mini_dist_shift.tex <==
\begin{table}[t]
%\vspace{-0.02in}
\captionof{table}{Average precision (AP) on the PASCAL VOC detection task. We use DeiT-T backbone on top of the YOLOv3 framework. We train YOLOv3 three times and report the average and standard deviation. Bold denotes the best results. OAMixer improves the detection performance.
}\label{tab:detection}
\centering\small
\resizebox{.45\textwidth}{!}{% 
\begin{tabular}{lccc}
\toprule
Backbone & AP25 & AP50 & AP75 \\
\midrule
% DeiT-S         & 1.57 & 0.78 & 0.95 & 0.29 \\
% MLP-Mixer-S/16 & 0.74 & 0.00 & 0.00 & 0.06 \\
% ConvMixer-S/16 & 0.87 & 2.35 & 1.50 & 0.00 \\
DeiT-T         & $40.02 \pm 0.38$ & $29.27 \pm 0.64$ & $0.08  \pm 0.01$ \\
+ OAMixer (ours) & \textbf{$42.54 \pm 0.27$} & $30.67 \pm 0.45$ & $0.08 \pm 0.01$ \\
\bottomrule
\end{tabular}}
%\vspace{-0.02in}
\end{table}




==> _cvprw2022_(arxiv)/resources/tab_more_classification_in_domain.tex <==
\begin{table}[t]
\caption{
Classification accuracy on various datasets. We add OAMixer to the baseline models using ReLabel trained on each downstream dataset. Bold denotes the best result, and parenthesis denotes the gap from the baseline. OAMixer gives a consistent improvement over various datasets.
}\label{tab:cls-more-in-domain}
% \vspace{-0.08in}
\centering\small
\resizebox{0.47\textwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
& \multicolumn{2}{c}{DeiT-T} & \multicolumn{2}{c}{DeiT-S} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5} 
& Baseline & OAMixer (ours) & Baseline & OAMixer (ours) \\
\midrule
CIFAR-10  & 86.35 & \textbf{89.89} \up{3.54} & 90.80 & \textbf{92.73} \up{1.93}\\
CIFAR-100 & 65.21 & \textbf{66.94} \up{1.73} & 70.08 & \textbf{71.00} \up{0.92} \\
Food-101  & 69.83 & \textbf{72.25} \up{2.42} & 75.00 & \textbf{75.17} \up{0.17}\\
Pets & 24.20 & \textbf{24.50} \up{0.30} & 25.57 & \textbf{30.64} \up{5.07} \\
\bottomrule
\end{tabular}}
\end{table}

==> _cvprw2022_(arxiv)/resources/tab_pascal.tex <==
\begin{table}[t]
%\vspace{-0.02in}
\captionof{table}{Average precision (AP) on the PASCAL VOC detection task. We use DeiT-T backbone on top of the YOLOv3 framework. We train YOLOv3 three times and report the average and standard deviation. Bold denotes the best results. OAMixer improves the detection performance.
}\label{tab:detection}
\centering\small
\resizebox{.45\textwidth}{!}{% 
\begin{tabular}{lccc}
\toprule
Backbone & AP25 & AP50 & AP75 \\
\midrule
% DeiT-S         & 1.57 & 0.78 & 0.95 & 0.29 \\
% MLP-Mixer-S/16 & 0.74 & 0.00 & 0.00 & 0.06 \\
% ConvMixer-S/16 & 0.87 & 2.35 & 1.50 & 0.00 \\
DeiT-T         & $40.02 \pm 0.38$ & $29.27 \pm 0.64$ & $0.08  \pm 0.01$ \\
+ OAMixer (ours) & \textbf{$42.54 \pm 0.27$} & $30.67 \pm 0.45$ & $0.08 \pm 0.01$ \\
\bottomrule
\end{tabular}}
%\vspace{-0.02in}
\end{table}




==> resources/fig_mixing.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}{0.28\textwidth}
\includegraphics[width=\textwidth]{figures/attn.png}
\caption{Self-attention}
\end{subfigure}
\begin{subfigure}{0.28\textwidth}
\includegraphics[width=\textwidth]{figures/mlp.png}
\caption{Feed-forward}
\end{subfigure}
\begin{subfigure}{0.28\textwidth}
\includegraphics[width=\textwidth]{figures/conv.png}
\caption{Convolution}
\end{subfigure}
\caption{
Illustration of representative patch mixing layers $f_\texttt{mix}$: (a) self-attention, (b) feed-forward, and (c) convolution. All layers map $N$ input patches to $N$ output patches, updating the values by interacting among the patches.
}\label{fig:mixing}
\end{figure*}




==> resources/tab_dist_shift_summary.tex <==
\begin{table}[t]
\caption{
sss
}\label{tab:dist-shift-summary}
% \vspace{-0.08in}
\centering\small
% \resizebox{0.7\textwidth}{!}{%
\begin{tabular}{cccc}
\toprule
\multicolumn{2}{c}{DeiT-T} & \multicolumn{2}{c}{DeiT-S} \\
\cmidrule(lr){1-2}\cmidrule(lr){3-4} 
Baseline & OAMixer (ours) & Baseline & OAMixer (ours) \\
\midrule
57.42 & \textbf{59.56} \up{2.14} & 60.93 & \textbf{62.23} \up{1.30} \\
\bottomrule
\end{tabular}%}
\end{table}

==> resources/tab_mask_scale.tex <==
\begin{table*}[t]
\begin{minipage}{0.48\textwidth}
\captionof{table}{
Learned mask scales $\kappa^{(l)}$ over layers.
}\label{tab:mask-scale}
%\vspace{-0.08in}
\resizebox{\textwidth}{!}{% 
\begin{tabular}{lcccc}
\toprule
& Layer 1/4 & Layer 2/4 & Layer 3/4 & Layer 4/4 \\
\midrule
DeiT-S         & 1.571 & 0.783 & 0.945 & 0.287 \\
MLP-Mixer-S/16 & 0.744 & 0.000 & 0.001 & 0.061 \\
ConvMixer-S/16 & 0.871 & 2.347 & 1.498 & 0.001 \\
\bottomrule
\end{tabular}}
\end{minipage}~~~~
\begin{minipage}{0.38\textwidth}
\centering
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/saliency_orig.png}
\caption{Original}
\end{subfigure}~
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/saliency_base.png}
\caption{DeiT-S}
\end{subfigure}~
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/saliency_ours.png}
\caption{OAMixer}
\end{subfigure}
%\vspace{-0.05in}
\captionof{figure}{
Saliency map visualization.
}\label{fig:saliency}
\end{minipage}
\end{table*}




==> resources/tab_mini_dist_shift.tex <==
\begin{table}[t]
%\vspace{-0.02in}
\captionof{table}{Average precision (AP) on the PASCAL VOC detection task. We use DeiT-T backbone on top of the YOLOv3 framework. We train YOLOv3 three times and report the average and standard deviation. Bold denotes the best results. OAMixer improves the detection performance.
}\label{tab:detection}
\centering\small
\resizebox{.45\textwidth}{!}{% 
\begin{tabular}{lccc}
\toprule
Backbone & AP25 & AP50 & AP75 \\
\midrule
% DeiT-S         & 1.57 & 0.78 & 0.95 & 0.29 \\
% MLP-Mixer-S/16 & 0.74 & 0.00 & 0.00 & 0.06 \\
% ConvMixer-S/16 & 0.87 & 2.35 & 1.50 & 0.00 \\
DeiT-T         & $40.02 \pm 0.38$ & $29.27 \pm 0.64$ & $0.08  \pm 0.01$ \\
+ OAMixer (ours) & \textbf{$42.54 \pm 0.27$} & $30.67 \pm 0.45$ & $0.08 \pm 0.01$ \\
\bottomrule
\end{tabular}}
%\vspace{-0.02in}
\end{table}




==> resources/tab_more_classification_in_domain.tex <==
\begin{table}[t]
\caption{
Classification accuracy on various datasets. We add OAMixer to the baseline models using ReLabel trained on each downstream dataset. Bold denotes the best result, and parenthesis denotes the gap from the baseline. OAMixer gives a consistent improvement over various datasets.
}\label{tab:cls-more-in-domain}
% \vspace{-0.08in}
\centering\small
\resizebox{0.47\textwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
& \multicolumn{2}{c}{DeiT-T} & \multicolumn{2}{c}{DeiT-S} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5} 
& Baseline & OAMixer (ours) & Baseline & OAMixer (ours) \\
\midrule
CIFAR-10  & 86.35 & \textbf{89.89} \up{3.54} & 90.80 & \textbf{92.73} \up{1.93}\\
CIFAR-100 & 65.21 & \textbf{66.94} \up{1.73} & 70.08 & \textbf{71.00} \up{0.92} \\
Food-101  & 69.83 & \textbf{72.25} \up{2.42} & 75.00 & \textbf{75.17} \up{0.17}\\
Pets & 24.20 & \textbf{24.50} \up{0.30} & 25.57 & \textbf{30.64} \up{5.07} \\
\bottomrule
\end{tabular}}
\end{table}

==> resources/tab_pascal.tex <==
\begin{table}[t]
%\vspace{-0.02in}
\captionof{table}{Average precision (AP) on the PASCAL VOC detection task. We use DeiT-T backbone on top of the YOLOv3 framework. We train YOLOv3 three times and report the average and standard deviation. Bold denotes the best results. OAMixer improves the detection performance.
}\label{tab:detection}
\centering\small
\resizebox{.45\textwidth}{!}{% 
\begin{tabular}{lccc}
\toprule
Backbone & AP25 & AP50 & AP75 \\
\midrule
% DeiT-S         & 1.57 & 0.78 & 0.95 & 0.29 \\
% MLP-Mixer-S/16 & 0.74 & 0.00 & 0.00 & 0.06 \\
% ConvMixer-S/16 & 0.87 & 2.35 & 1.50 & 0.00 \\
DeiT-T         & $40.02 \pm 0.38$ & $29.27 \pm 0.64$ & $0.08  \pm 0.01$ \\
+ OAMixer (ours) & \textbf{$42.54 \pm 0.27$} & $30.67 \pm 0.45$ & $0.08 \pm 0.01$ \\
\bottomrule
\end{tabular}}
%\vspace{-0.02in}
\end{table}



